A Survey on Ransomware: Evolution, Taxonomy, and Defense Solutions

In recent years, ransomware has been one of the most notorious malware targeting end users, governments, and business organizations. It has become a very profitable business for cybercriminals with revenues of millions of dollars, and a very serious threat to organizations with financial loss of billions of dollars. Numerous studies were proposed to address the ransomware threat, including surveys that cover certain aspects of ransomware research. However, no study exists in the literature that gives the complete picture on ransomware and ransomware defense research with respect to the diversity of targeted platforms. Since ransomware is already prevalent in PCs/workstations/desktops/laptops, is becoming more prevalent in mobile devices, and has already hit IoT/CPS recently, and will likely grow further in the IoT/CPS domain very soon, understanding ransomware and analyzing defense mechanisms with respect to target platforms is becoming more imperative. In order to fill this gap and motivate further research, in this paper, we present a comprehensive survey on ransomware and ransomware defense research with respect to PCs/workstations, mobile devices, and IoT/CPS platforms. Specifically, covering 137 studies over the period of 1990-2020, we give a detailed overview of ransomware evolution, comprehensively analyze the key building blocks of ransomware, present a taxonomy of notable ransomware families, and provide an extensive overview of ransomware defense research (i.e., analysis, detection, and recovery) with respect to platforms of PCs/workstations, mobile devices, and IoT/CPS. Moreover, we derive an extensive list of open issues for future ransomware research. We believe this survey will motivate further research by giving a complete picture on state-of-the-art ransomware research.

==> backup.tex <==







\twocolumn
  \LTcapwidth=\textwidth
  \renewcommand\arraystretch{1}
  \begin{longtable}
  {|>{\footnotesize}p{2cm}|>{\footnotesize}p{1.5cm}|>{\footnotesize}p{2cm}|>{\footnotesize}p{2cm}|>{\footnotesize}p{1.3cm}|>{\footnotesize}p{0.7cm}|>{\footnotesize}p{0.7cm}|>{\footnotesize}p{0.7cm}|>{\footnotesize}p{0.8cm}|>{\footnotesize}p{0.8cm}|}\caption{Summary of Android Defense Systems}\label{tab:iiot-cps-honeypots-tools} \hline
  
 
    %\begin{tabular}{|p{11.59em}|c|p{5.455em}|p{3.955em}|p{5.365em}|p{23.59em}|p{3.18em}|p{3.32em}|p{4.365em}|}
    %\toprule
    \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Work}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Target}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Features}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\parbox{2cm}{\centering\textbf{Detection Technique}}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\parbox{1.3cm}{\centering \textbf{Recovery Support}}}} &
  \multicolumn{3}{c|}{\textbf{Dataset}} &
  \multicolumn{2}{c|}{\textbf{Performance}} \\ \cline{6-10} 
 &   &  & & & \multicolumn{1}{c|}{\textbf{Families}} &
  \multicolumn{1}{c|}{\textbf{Samples}} &
  \multicolumn{1}{c|}{\textbf{Benign}} &
  \multicolumn{1}{c|}{\textbf{TPR}} &
  \multicolumn{1}{c|}{\textbf{FPR}} \\\endfirsthead \hline
    
\multicolumn{6}{c}{\tablename\ \thetable: Summary of Ransomware Defense Research (Cont.)} \\
\hline
  \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Work}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Target}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Features}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\parbox{2cm}{\centering\textbf{Detection Technique}}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\parbox{1.3cm}{\centering \textbf{Recovery Support}}}} &
  \multicolumn{3}{c|}{\textbf{Dataset}} &
  \multicolumn{2}{c|}{\textbf{Performance}} \\ \cline{6-10} 
 &   &  & & & \multicolumn{1}{c|}{\textbf{Families}} &
  \multicolumn{1}{c|}{\textbf{Samples}} &
  \multicolumn{1}{c|}{\textbf{Benign}} &
  \multicolumn{1}{c|}{\textbf{TPR}} &
  \multicolumn{1}{c|}{\textbf{FPR}}\\\endhead \hline
   
    
GreatEatlon \cite{greatEeatlon} & Cryptographic & API Calls,permissions,package names, APK informations  & Static Behavior &  &- &75&-&99& \simeq 0 \\\hline



\textbf{HelDroid} \cite{HelDroid} &Android & APK Analysis & Signature Based &  & &650 &81046&99 & \simeq 0 \\\hline


\textbf{DNADroid} \cite{DNADROID} &Android All & API Calls, Strings & Machine-Learned &  &8 &1928&2500&97.5&\simeq 0.5  \\\hline
\textbf{Karimi et al.} \cite{Karimietal} &Android Locker & APK Analysis & Machine-Learned & - &3 &250&30 &97.5& - \\\hline
\textbf{R-packDroid} \cite{R-Pack} &Android All & API Calls, Strings & Machine-Learned &  &- &2,047&4,098&97& 1 \\\hline

\textbf{Chen et al.} \textbf{R-packDroid} \cite{flowgraph} &Cryptographic& API calls (CFG)& Machine-Learned(Logistic Regression) &  & 4&83&85&97.6& 1.2 \\\hline

\textbf{Cuzzocrea et al.}  \cite{stractrualEntropy} &All&  Entropy of Apps & Machine-Learned(Fuzzy logic) &  & &2052& 10,000 &83& 19 \\\hline
\textbf{EliteApp} \cite{eliteApp} &Locker& permissions, image, file & APK anaylysis &  & &-& - &-& - \\\hline

\textbf{RansomProber}  \cite{real-timeAndroid} &Cryptographic&File List, Hint Text button& UI Analysis & -&15&2,721 &9,238 &99& - \\\hline

\textbf{Alsoghyer et al. }  \cite{Alsoghyer_2019} & Locker &API Calls & Machine-Learned(RF)& -&-&500 &500 &94& \simeq 3 \\\hline


\textbf{Ferrante et al.  }  \cite{ferrante} & All&2-grams opcode, CPU,Network,Memory usage, system call statistics &Hybrid Analysis & -&-&672 &2,386 &100& \simeq 4 \\\hline



\textbf{Alzahrani et al.  }  \cite{alzahrani} & All &APIs, Intends, permissions &Machine-Learned (RF)  & -&10&259 &200 &96& 1.64 \\\hline

\textbf{Scalas et al. } \cite{effectofAPIAndroid} & All &APIs &Machine-Learned (RF)  & -&- &3017 &200 &97& 1 \\\hline

\textbf{Bibi et al.  } \cite{AndroidDeep} &All   &Permissions &Machine-Learned (DL)  & -&- &500 &500 &97.08& 3.1 \\\hline

\textbf{Faris et al.  }  \cite{Farisetal} &Android & API calls, permissions   &Machine-Learned& - &- &500&500 & 98& 0.2 \\\hline


\textbf{Lachtar et al. } \cite{nativeMobile} & Android   & Native instructions opcodes &Machine-Learned(RF)   & -&- &2148 &- &99.8& 0 \\\hline


\textbf{Alsoghyer et al.  } \cite{permissionsAndroid} &All   &Permissions &Machine-Learned (RF)  & -&- &500 &500 &96.9& 3.1 \\\hline


\textbf{Nikolai et al. } \cite{Nikolai_2016} & Android   &Formal Methods &Static  & -&- &683 & 600 &99 & \simeq 0  \\\hline
 
 
\textbf{TALOS } \cite{TalosNM} & Android   &Formal Methods &Static  & -&- &683 & 1500 &99 & 0.5 \\\hline
 
 
 
\textbf{RANSOMSAFEDROID } \cite{yalewetal} & Android   &Back-up &  & -&- &683 & 1500 &99 & 0.5 \\\hline

\textcolor{red}{MimosaFTL  } \cite{mimosaFTL} & Android Recovery  &
I/O Flash Storage &Hardware-Assisted &\checkmark &11&346&95 & \simeq 100 & 0 \\\hline

 

\end{longtable}

\twocolumn



\twocolumn
  \LTcapwidth=\textwidth
  \renewcommand\arraystretch{1}
  \begin{longtable}
  {|>{\footnotesize}p{2cm}|>{\footnotesize}p{1.5cm}|>{\footnotesize}p{2cm}|>{\footnotesize}p{2cm}|>{\footnotesize}p{1.3cm}|>{\footnotesize}p{0.7cm}|>{\footnotesize}p{0.7cm}|>{\footnotesize}p{0.7cm}|>{\footnotesize}p{0.8cm}|>{\footnotesize}p{0.8cm}|}\caption{Summary of Personal Computer Defense Systems}\label{tab:iiot-cps-honeypots-tools} \hline
  
 
    %\begin{tabular}{|p{11.59em}|c|p{5.455em}|p{3.955em}|p{5.365em}|p{23.59em}|p{3.18em}|p{3.32em}|p{4.365em}|}
    %\toprule
    \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Work}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Target}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Features}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\parbox{2cm}{\centering\textbf{Detection Technique}}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\parbox{1.3cm}{\centering \textbf{Recovery Support}}}} &
  \multicolumn{3}{c|}{\textbf{Dataset}} &
  \multicolumn{2}{c|}{\textbf{Performance}} \\ \cline{6-10} 
 &   &  & & & \multicolumn{1}{c|}{\textbf{Families}} &
  \multicolumn{1}{c|}{\textbf{Samples}} &
  \multicolumn{1}{c|}{\textbf{Benign}} &
  \multicolumn{1}{c|}{\textbf{TPR}} &
  \multicolumn{1}{c|}{\textbf{FPR}} \\\endfirsthead \hline
    
\multicolumn{6}{c}{\tablename\ \thetable: Summary of Ransomware Defense Research (Cont.)} \\
\hline
  \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Work}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Target}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Features}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\parbox{2cm}{\centering\textbf{Detection Technique}}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\parbox{1.3cm}{\centering \textbf{Recovery Support}}}} &
  \multicolumn{3}{c|}{\textbf{Dataset}} &
  \multicolumn{2}{c|}{\textbf{Performance}} \\ \cline{6-10} 
 &   &  & & & \multicolumn{1}{c|}{\textbf{Families}} &
  \multicolumn{1}{c|}{\textbf{Samples}} &
  \multicolumn{1}{c|}{\textbf{Benign}} &
  \multicolumn{1}{c|}{\textbf{TPR}} &
  \multicolumn{1}{c|}{\textbf{FPR}}\\\endhead \hline
   
    
\textbf{UNVEIL} \cite{EnginKirda} & - & File system access patterns, I/O Data Buffer Entropy & (File) System-Behavior&  &15 &2,201&49&96.3&0 \\\hline


\textbf{CryptoDrop} \cite{cryptoDrop} & -& File type changes and funneling,Similarity Measurement, Shannon Entropy & (File) System-Behavior & - &14 &492&30&100&1 \\\hline
\textbf{SHIELDFS} \cite{shieldFS} & -  & Folder-listing, Files-Read/Written/Renamed, File type coverage, Write-Entropy  & File Activity Behavior Machine-Learned (RF)  & Symmetric key & 18 &688&2245&97.7&0.038 \\\hline


\textbf{Palisse et al. } \cite{DaD} & - &
Write and Information Operations, Central Tendency& File System Behavior & - & 15 &8,152&1000 & 98.8 & 7.1 \\\hline



\textbf{CloudRPS } \cite{cloudEnhanced} & All &
Server,file, network & Monitoring & Back-up &- &-  & - & - & \\\hline

\textbf{RWGuard} \cite{RWGuard} & - & Processes, File Changes & Machine-Learned(RF) & Crypto Hooking & 14&14&261&100&\simeq0.1 \\\hline




\textbf{REDEMPTION} \cite{redemption} & - & Entropy Ratio of Data Blocks, File Content Overwrite, Delete Operation,Directory Travers, Converting to a Specific File Type ,Access Frequency & (Process)Behavior-Based &every write request to a sparse file in a protected area without
changing the original file. & 29&1,181 &230GB&100&0.8 \\\hline





\textbf{GURLS} \cite{Gurls} & - & Strings, Frequency of API Calls & API Calls with GURLS  &  &10 &268&66&87.7& 7.5 \\\hline


\textbf{Takeuchi et al.}\cite{SVMBased} & - & API calls & Machine-Learned (SVM) &  &276&312&-&97.48&1.64  \\\hline


\textbf{Zhou et al.}  \cite{correlations} &All&Correlations between APIs &Machine-Learned(SVM)& - &9&150&899&98&- \\\hline


\textbf{Maniath et al.}  \cite{lstmbased} & - &  API Calls & Deep-Learned (LSTM) &  &- &157&-&96,67& - \\\hline

\textbf{Agrawal et al. } \cite{recurrentNeural} & -   &
API Calls &Deep-Learned(LSTM) &- &-&26300 & & 93 & 2 \\\hline



Vinayakumar et al.\cite{shallowDeep} &Cryptographic & API Calls & Deep-Learned &  -&7 &755&219&98& \simeq 0.5 \\\hline


\textbf{Maroof et al.  } \cite{zeroDayAware} &Cryptographic &API-gram & Machine-Learned(SVM) & - &4 &38,152&1000&99& 2.4 \\\hline


\textbf{Al-rimy et al.  } \cite{al-rimy} &PC &
API calls & Machine-learned & - & 15 &8,152&1000 & 98.8 & 7.1 \\\hline

\textbf{2entFOX} \cite{2EntFox} & HSRs &Registry Operations, File, directory accesses  & Machine-Learned &  & 8 &8&8&100&0 \\\hline


\textbf{Chang et al. } \cite{chang:2019}  &HSR& IP Addresses & Network Analysis(KNN) &  &-&-&-&76.5& 3 \\\hline



\textbf{Abukar et al.} \cite{HSRAutomated}  &HSR& Registry paths,API Calls, Directory-File Operations, Cryptographic libraries & Machine-Learned(ANN) &  &14 &1254&1308&98.6& 2.6 \\\hline

Akbano \cite{wannaCRYSDN} &  WannaCry & Flow features& Network-Monitoring&  & 1 &-&-&-&- \\\hline

Wani et al. \cite{wanietal.} & SDN-based crypto & Flow features& Network-Monitoring &  & 1 &78&-&98&2.1 \\\hline


REDFISH \cite{redFish} & Network-Encrypted & number of bytes R/W, file content& Network-Monitoring&  & 19 &54&30&100&\simeq0 \\\hline

\textbf{Hwang et al. }  \cite{twoStageML} &Cryptographic &API Calls, strings, registry, file system directory operations. &System-behavior& - &-&1176&1160&97&\simeq 4.83 \\\hline
\textbf{Khan et al. }  \cite{DNA-Sequencing} &All&API Calls, strings, registry, file system directory operations. &Machine-Learned& - &11&150&150&87.9&\simeq 10 \\\hline


\textbf{Jethva et al. } \cite{Jethvaetal} &All   &
API calls, grouped registry key operations, Windows DLLs, directory, enumerations, embedded strings &Machine-Learned (SVM)  & -&20 &666&103& \simeq 100& 1.41 \\\hline





\textbf{RANSHUNT}  \cite{ransHaunt} &Cryptographic & API calls, registry key ,file system,process and network  & Machine-Learned &  & 21&360&460&97.1& \simeq 3 \\\hline

Chen et al. \cite{chenetal} &Cryptographic & -  & Machine-Learned &  & -&83&85&97.6& $\simeq$1.2 \\\hline
\textbf{EldeRan} \cite{eldeRan} &Cryptographic & API stats, registry key operations, file directory operations, strings & Machine-Learned (Logistic Regression) &  & 11&582&942&96.3&1.6 \\\hline 
Cusack et al. \cite{cusac} &Cryptographic & network traffic traces & Network-analysis based &  &- &100MB&100MB&87&10 \\\hline
\textbf{RansomWall} \cite{ransomwall} &Cryptographic & PE,entropy,strings,file- system operations & Machine-Learned& File-Backup Layer &12 &574&442&98.25&\simeq 0 \\\hline
DeepRan \cite{DeepRan} &Cryptographic &process information, opcode, event informations & Machine-Learned &  &17 &929,967&4.820&99.87& 0 \\\hline




\textbf{Medhat et al.} \cite{medhatetal} &Cryptographic & API functions, keywords, cryptography signatures,extensions &Static analysis /signatures &  -&45&793&878&98.3&8.4  \\\hline
Zhanga et al. \cite{ZHANG2020708} &Cryptographic & -  & Machine-Learned &  &17 &302&-&97&  \\\hline
\textbf{Zhang et al. }\cite{ZHANG2019211} &All & N-grams  & Machine-Learned(Random Forest) &  &8 &1787&-&99.8& - \\\hline
\textbf{Baldwin et al. }\cite{SVMbaldwin} &Cryptographic & Opcode & Machine-Learned(SVM) &  &5&5&1&97.1& 0.3 \\\hline


\textbf{SVM et al. }\cite{SVMbaldwin} &Cryptographic & Opcode & Machine-Learned(SVM) &  &5&5&1&97.1& 0.3 \\\hline



\textbf{Jung et al. } \cite{jung:2018} &Cryptographic & Read/Write logs & File System Activity & Secure Zone &- &-&-&-& - \\\hline


\textbf{NETCONVERSE  } \cite{Alhawi2018} &All &Network Traffic & Machine-Learned(DT) & - &9&210&264&95& \simeq 3.5 \\\hline


\textbf{Poudyal et al. } \cite{poudyaletal} &All &Assembly, DLL level code & Machine-Learned(RF) & - &12&178&178&97& - \\\hline


\textbf{CRED } \cite{VectorSpace} &All & APIs, I/O Sequences&  Machine-Learned(LSTM) & - &-&-&-&-& - \\\hline
\textbf{Islam et al. } \cite{patternExtraction} & Cryptographic& API calls, files,registry keys, Mutexes,Network traffic & Machine-Learned &-&7&7&-&99& 0 \\\hline

\textbf{Gangwar et al. }  \cite{DetectionViaInfection} &Cryptographic &Redirection Count, IP addresses, File Types& Machine-Learned(NaiveBayes)  & - &-&50&50&97& 0.02 \\\hline

\textbf{Arivudainambi }  \cite{Arivudainambi:2020} &Cryptographic &Network Traffic &Deep-Learned & - &3&45678&-&96.5& -\\\hline





\textbf{Dash et al. }  \cite{IoTDetectML} &IoT & Network Traffic &Machine-Learned(KNN)&  &- &- &- &93.76&- \\\hline

\textbf{Bae et al.  }  \cite{Baeetal.} &Cryptographic & API Calls  &Machine-Learned& - &58 &1000 & 300 & \simeq 98 & \\\hline




\textbf{Hawawreh et al.  }  \cite{deepIoT} &IoT& API calls,registry keys,file and directory operaitons &Machine-Learned& - &- &582&942 & 92.53& 7.47 \\\hline



\textbf{Goya et al.  }  \cite{Goyal:2020} &Cryptographic& high generation rate of encrypted files, high file write operations, high CPU utilization, deleting shadow copies, changing registries, renaming files, increasing size of files, changing wallpaper and network activity &Behavior-Based& - &5 &200& 'many' & 95 & 0 \\\hline



\textbf{Taylor et al.  }  \cite{Taylor2017SensorbasedRD} &Cryptographic & Sensor based monitoring &Machine-Learned& - &1& 1& & 95 &  \\\hline

\textbf{Zuhair et al. }  \cite{zuhairetal} &All & File related features, API calls, registry key, PE header, Shannon's entropy, Embedded Scripts &Machine-Learned& - &14& 35,000&500 & 97 &2.4 \\\hline

\textbf{Modi et al.  }  \cite{modi:2020} &Cryptographic &Communications Certifications &Network-Behavior& - &20& 666 &30 & 99 &0 \\\hline


\textbf{Sharmeen et al. }  \cite{avoidingDigital} &All  &API Calls  &Machine-Learned(Semi-Supervised)& - &14& 1232 &1308 & 94.61 &5.38 \\\hline

\textbf{Abbasi et al. }  \cite{Abbasietal} &All  & API, file directory operations strings, file extensions & Machine-Learned(wrapper based )& - &11& 582 &942 & \simeq 97.34 &- \\\hline




\textbf{Saleh et al. } \cite{salehetal} &All   &Assembly language Instructions &Machine-Learned (HMM)  & -&- &17&19 &73& - \\\hline


\textbf{Ashraf et al. } \cite{Ashrafetal} &All   &PE Header, Strings, File,Registry changes, API calls, DLLs, Extensions & Machine-Learned (ResNet-18)  & -&- &45,000&3000 & \simeq 92 & \simeq 3  \\\hline



\textbf{Egunjobi et al. } \cite{Egunjobietal} &All   &
hash value, file size, dll calls, mutexes, pe info&Machine-Learned (SVM)  & -&- &200&200& 100&  1 \\\hline


\textbf{Martinelli et al. } \cite{Martinelli2018PhylogeneticAF} &All   &
API Calls & Machine-Learned &- &3&91&100& 88.5 &  16.9 \\\hline



\textbf{Arabo et al. } \cite{araboetal} &All   &
Processes & Machine-Learned &- &3&91&100& 88.5 &  16.9 \\\hline





\textbf{Lemmout et al. } \cite{lemmouetal.} &All   &
Strings,  Memory snapshots & Behavior-based(Distance) &- &-&365&110000(T)& 96.05 &  0 \\\hline



\textbf{Cohen et al. } \cite{COHEN2018158} &All   &
DLL, Process, Mutex, Processes& Behavior-based(MemoryML) &- &5&100&100& 99 &  8 \\\hline



\textbf{Park et al. } \cite{RansomBlocker} &All   &
DLL, Process, Mutex, Processes& Hardware-Assisted&\checkmark&3&3&- & 100 & 0 \\\hline

\textcolor{red}{MimosaFTL  } \cite{mimosaFTL} &All   &
I/O Flash Storage &Hardware-Assisted &\checkmark &11&346&95 & \simeq 100 & 0 \\\hline


\textcolor{red}{FlashGuard } \cite{flashGuard} & Cryptographic  &
-  &Hardware-Assisted &\checkmark & & &  &  100 & 0 \\\hline

\textcolor{red}{SSD-Insider  } \cite{SSD_Insider} & Cryptographic   &
I/O Flash Storage &Hardware-Assisted + Behavior Based &\checkmark & & & & 100 & \simeq 0 \\\hline



\textbf{Maimo et al.} \cite{clinicalEnv} &All   &
Network Flow data &Machine-Learned(DT)  & - & &26300 & & 97 & 2 \\\hline


\textbf{DRTHIS } \cite{DRTHIS} &All   &
Network Flow data &Deep-Learned(LSTM)  & - & 3 &660&219 & 97.2 & 0 \\\hline


\textbf{Lu et al. } \cite{Luetal} & All  &
API call sequences & Negative Selection Algorithm & - & - &2000&1000 & 96 & - \\\hline

\textbf{Sitnikova et al. } \cite{IoTStacked} &IoT &
Registry keys, File-Directory operations, API calls &Deep-Learned & - & - &582&942 & 99.47 & 13.9 \\\hline


\textbf{Lee et al. } \cite{movingTarget} & PC &
 - & Extension randomization & - & 6 & 143  &-  & 98.6 & - \\\hline



DIMAQS \cite{databasedetect} & Server-side&
Queries & Colered Petrinets  & - & - &-  &- & 100 & 0 \\\hline


\textbf{Homayoun et al. } \cite{KnowAbnormal.} & PC &
Registry, File Operations, DLL & Machine-learned (RF) & - & 3 &1624 &220 & 99.4 & 4 \\\hline

\textbf{Amoeba } \cite{minetal} & PC &
 -  & SSD-Based Recovery & 3 &1624 &220 & 99.4 & 2.57 \\\hline


\textbf{Ahmed et al.  } \cite{AHMED2020102753} & PC &
 API Calls  & Machine Learned & 14 &1354 &1358 & 97.4 & 1.6 \\\hline



\textbf{Migi et al. } \cite{migidaetal} &All   &
API Calls, registry key operations, embedded strings and file related features,extension of the drop files,file directory operations  & Machine-Learned &- & 11 &582 &942& 99.7 &  \simeq 0.1 \\\hline
\end{longtable}

\twocolumn








 

